Experimental study of perovskite nanocrystals as single photon sources for integrated quantum photonics

This thesis is devoted to the study of the coupling of single-photon emitters with photonic nanostructures by using the properties of the near field of a photonic structure in view of the realization of a compact integrated single-photon source for quantum applications. The first part of my thesis work was consecrated to the optimization of perovskites nanocrystals. Although perovskites nanocrystals are very promising single-photon sources, they still need improvements: in this work, I review the main properties of these emitters and present a full characterization of perovskite nanocrystals with improved photo-stability, reduced blinking ad strong antibunching. In the second part of the thesis, I focus on the coupling of quantum emitters with various photonic structures: namely the tapered optical nanofibers and the ion-exchange waveguides. The fabrication method and the optical properties of the nanofibers are described in detail and the coupling of a single perovskite nanocrystal with a nanofiber is achieved, which constitutes a proof of principle of a hybrid integrated single-photon source. Finally, I show how the near field around ion exchange waveguides can be employed together with near-field polymerization to trap single-photon emitters onto the waveguides.

==> thcoverdata.tex <==
%!TeX encoding = UTF-8
% Metadata for coverpages
\thesisname{Thèse de doctorat}
\gradename{docteur}
\univ{de l'Université de Technologie de Troyes}
%\logos{Logos/Logo_of_Sorbonne_University.pdf}{Logos/LKB.pdf}{Logos/ICD.pdf}
\logosf{Logos/ICD.pdf}{Logos/logol2nessai4a.pdf}{Logos/LKB.pdf}{Logos/Logo_of_Sorbonne_University.pdf}
%{LKB}{LKB}                   %
%%Un à trois logo. Le 1er est
%%celui de
%\univ
\specialite{Matériaux, Mécanique, Optique et Nanotechnologie}
\ecoledoctnum{361}
\ecoledoct{Sciences pour l'Ingénieur}
\title{}
\titleen{Experimental study of perovskite nanocrystals as single photon sources
	for integrated quantum photonics}

% si nécessaire, pour les métadonnées
%\titlemeta{La laine des Dupondt au Pays de l'or noir}
%\titlemetaen{Dupondt's wool in "Land of Black Gold" }

\date{27/11/2020}
\author{Stefano PIERINI}
\advisor{Christophe COUTEAU et Alberto BRAMATI}
\atinstitution{à l'Universitè de Technologie de Troyes}
\atlab{{\Large à l'Institut Charles Delaunay et au Laboratoire Kastler Brossel}}
% Jury as LaTeX Tabular. Pas de président avant soutenance
\jury{ %
Mme & Carole DIEDERICHS& Rapporteur        \\
M. & Marco GENOVESE & Rapporteur        \\
Mme & Sara DUCCI & Examinatrice           \\
M. & Alberto BRAMATI & Directeur de thèse      \\
M. & Christophe COUTEAU & Directeur de thèse      \\
M. & Emmanuel LHUILLIER & Invité}
\makeatletter
\@ifpackageloaded{thcover-psl}{\logos{PSL}{LKB}{}}{\relax}
\makeatother

\resume{
}

\motscles{}

% si nécessaire, pour les métadonnées
%\titlemetaen{Dupondt's wool in "Land of Black Gold" }

\abstract{
}

\keywords{}


